Deep Reinforcement Learning based Blind mmWave MIMO Beam Alignment

Directional beamforming is a crucial component for realizing robust wireless communication systems using millimeter wave (mmWave) technology. Beam alignment using brute-force search of the space introduces time overhead while location aided blind beam alignment adds additional hardware requirements to the system. In this paper, we introduce a method for blind beam alignment based on the RF fingerprints of user equipment obtained by the base stations. The proposed system performs blind beam alignment on a multiple base station cellular environment with multiple mobile users using deep reinforcement learning. We present a novel neural network architecture that can handle a mix of both continuous and discrete actions and use policy gradient methods to train the model. Our results show that the proposed method can achieve a data rate of up to four times the traditional method without any overheads.

==> figs/basestation.tex <==

% chktex-file 1
% chktex-file 27

\makeatletter


% The keys that the user can provide are all the keys below.

% Keys for the Beam shape
\pgfkeys{
  /pgf/.cd,
  % The 4 following options control the proportion of shapewidth/shapeheight for
  % the control points of the beam -> The must be greater than zero
  control point 1 x/.initial=0.35,
  control point 1 y/.initial=1.0,
  control point 2 x/.initial=0.5,
  control point 2 y/.initial=0.25,
}

% Keys for the UserTerminal shape
\pgfkeys{
  /pgf/.cd,
  button fill color/.initial=white,
  screen fill color/.initial=white,
}


% Represents a "beam", which is constructed using two Bézier curves.
% The two control points can be controlled by passing the
% "control point 1 x/control point 1 y/control point 2 x/control point 2 y"
% parameters.
\pgfdeclareshape{Beam}{

  % xxxxxxxxxx Define some saved macros xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \savedmacro\shapewidth{
    \def\shapewidth{\pgfkeysvalueof{/pgf/minimum width}}
  }

  \savedmacro\shapeheight{
    \def\shapeheight{\pgfkeysvalueof{/pgf/minimum height}}
  }

  \savedmacro\firstpointxprop{
    \def\firstpointxprop{\pgfkeysvalueof{/pgf/control point 1 x}}
  }
  \savedmacro\firstpointyprop{
    \def\firstpointyprop{\pgfkeysvalueof{/pgf/control point 1 y}}
  }
  \savedmacro\secondpointxprop{
    \def\secondpointxprop{\pgfkeysvalueof{/pgf/control point 2 x}}
  }
  \savedmacro\secondpointyprop{
    \def\secondpointyprop{\pgfkeysvalueof{/pgf/control point 2 y}}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  \savedanchor\startpoint{%
    \pgfmathsetlength\pgf@x{-0.5*\shapewidth}
    \pgfmathsetlength\pgf@y{0}
  }

  \savedanchor\endpoint{%
    \pgfmathsetlength\pgf@x{0.5*\shapewidth}
    \pgfmathsetlength\pgf@y{0}
  }

  % \savedanchor\centerpoint{%
  %   \pgf@x=0%
  %   \pgf@y=0%
  % }

  % Control point anchors
  \savedanchor\firstcontrolpointtop{%
    \pgfmathsetlength\pgf@x{\firstpointxprop*\shapewidth}
    \pgfmathsetlength\pgf@y{\firstpointyprop*\shapeheight}
  }

  \savedanchor\secondcontrolpointtop{%
    \pgfmathsetlength\pgf@x{\secondpointxprop*\shapewidth}
    \pgfmathsetlength\pgf@y{\secondpointyprop*\shapeheight}
  }

  \savedanchor\firstcontrolpointbottom{%
    \pgfmathsetlength\pgf@x{\firstpointxprop*\shapewidth}
    \pgfmathsetlength\pgf@y{-\firstpointyprop*\shapeheight}
  }

  \savedanchor\secondcontrolpointbottom{%
    \pgfmathsetlength\pgf@x{\secondpointxprop*\shapewidth}
    \pgfmathsetlength\pgf@y{-\secondpointyprop*\shapeheight}
  }

  % xxxxxxxxxx Define regular anchors xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \anchor{center}{\startpoint}
  \anchor{start}{\startpoint}
  \anchor{end}{\endpoint}
  \anchor{main region}{
    \endpoint
    \pgfmathsetlength\pgf@x{\pgf@x-0.25*\shapewidth}
  }
  \anchor{top control point 1}{\firstcontrolpointtop}
  \anchor{top control point 2}{\secondcontrolpointtop}
  \anchor{bottom control point 1}{\firstcontrolpointbottom}
  \anchor{bottom control point 2}{\secondcontrolpointbottom}
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  \inheritanchorborder[from=rectangle]

  % xxxxxxxxxx Draw the background path xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \backgroundpath{
    \begin{pgfscope}
      \pgfmoveto{\startpoint}
      \pgfcurveto{\firstcontrolpointtop}{\secondcontrolpointtop}{\endpoint}
      \pgfcurveto{\secondcontrolpointbottom}{\firstcontrolpointbottom}{\startpoint}
      \pgfpathclose
      \pgfusepath{fill}
    \end{pgfscope}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
}


% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx UserTerminal Shape xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
\pgfdeclareshape{UserTerminal}{

  % xxxxxxxxxx First we define some savedmacros xxxxxxxxxxxxxxxxxxxxxxxxxxx
  % Macros and savedanchors common to UserTerminal and BaseStation Shapes
  \savedanchor{\center}{
    \pgf@x=0pt
    \pgf@y=0pt
  }

  % Note that pgf provides the text macros \pgfshapeminwidth and
  % pgfshapeminheight that store the minim width and minimum height,
  % respectivelly. Note that They are "TEXT macros" and not
  % "lengths". Calling them simple
  % replaces for the text.
  \savedanchor{\northeast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0.5\pgf@xa
    \pgf@y=0.5\pgf@ya
    % NOTE: We can't use 0.5\pgfshapeminwidth directly because the minimum
    % width is stored in a "plain text macro". If minimum width is 2cm, for
    % instance, and we write "\pgf@x=.5\pgfshapeminwidth" then \pgf@x would
    % be set to 0.52cm, which is not what we want. See the explanation for
    % \savedanchor in the pgfmanual (page 627).
  }

  \savedanchor{\southwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=-0.5\pgf@xa
    \pgf@y=-0.5\pgf@ya
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % Savedanchors specific to the UserTerminal shape
  \savedanchor{\screennortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0.45\pgf@xa
    \pgf@y=0.45\pgf@ya
  }

  \savedanchor{\screensouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=-0.45\pgf@xa
    \pgf@y=-0.35\pgf@ya
  }

  \savedanchor{\buttonsouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0pt
    \pgf@y=-0.425\pgf@ya
    \advance\pgf@x by -0.15\pgf@xa
    \advance\pgf@y by -0.04\pgf@ya
  }

  \savedanchor{\buttonnortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0pt
    \pgf@y=-0.425\pgf@ya
    \advance\pgf@x by 0.15\pgf@xa
    \advance\pgf@y by 0.04\pgf@ya
  }

  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit anchor border from rectangle xxxxxxxxxxxxxxxxxxxxxxx
  \inheritanchorborder[from=rectangle]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit normal anchors from rectangle xxxxxxxxxxxxxxxxxxxxxx
  % We define the savedanchors "northeast" and "southwest". With these two
  % defined we can inherit code for the regular anchors from the
  % rectangle shape (even thought the northeast and southwest saved anchors
  % in the rectangle shape are different from ours).
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Now we define more regular anchors xxxxxxxxxxxxxxxxxxxxxxxxx
  \anchor{text}
  {
    % This will get the center of the screen
    \pgfpointlineattime{0.5}{\screensouthwest}{\screennortheast}
    % Lets put the center of the text in the center of the screen
    \advance\pgf@x by -0.5\wd\pgfnodeparttextbox
    \advance\pgf@y by -0.5\ht\pgfnodeparttextbox
  }

  \anchor{button}{
    \pgfpointlineattime{0.5}{\buttonsouthwest}{\buttonnortheast}
  }

  \anchor{screen}{
    \pgfpointlineattime{0.5}{\screensouthwest}{\screennortheast}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Draw the background xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \backgroundpath{
    % Scope for Terminal Body
    \begin{pgfscope}
      \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
      % '\pgfshapeminheight' cannot be used directly; or if you want to use it directly use the '*' for multiplication
      \pgfsetcornersarced{\pgfpoint{0.03\pgf@ya}{0.03\pgf@ya}}
      \pgfpathrectanglecorners
      {\southwest}
      {\northeast}
      \pgfusepath{stroke,fill}
    \end{pgfscope}

    % Scope for the terminal Screen
    \begin{pgfscope}
      \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
      \pgfsetcornersarced{\pgfpoint{0.03\pgf@ya}{0.03\pgf@ya}}
      \pgfsetfillcolor{\pgfkeysvalueof{/pgf/screen fill color}}
      %\pgfsetfillcolor{white}
      \pgfpathrectanglecorners
      {\screensouthwest}
      {\screennortheast}
      \pgfusepath{stroke,fill}
    \end{pgfscope}

    % Scope for the button
    \begin{pgfscope}
      \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
      \pgfsetcornersarced{\pgfpoint{0.009\pgf@ya}{0.009\pgf@ya}}
      \pgfsetfillcolor{\pgfkeysvalueof{/pgf/button fill color}}
      %\pgfsetfillcolor{white}
      \pgfpathrectanglecorners
      {\buttonsouthwest}
      {\buttonnortheast}
      \pgfusepath{stroke,fill}
    \end{pgfscope}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
}
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx END xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx


% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx BaseStationSimple xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
\pgfdeclareshape{BaseStationSimple}{

  % xxxxxxxxxx Define savedanchors xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % Inherit all savedanchors from UserTerminal. We only need northeast and
  % southwest, but we can't choose which ones to inherit.
  \inheritsavedanchors[from=UserTerminal]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxx Define savedanchors specific to the BaseStation shape xxxxxxxxxxx
  \savedanchor{\BaseAsouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@y=-0.5\pgf@ya
    \pgf@x=-0.12\pgf@xa
  }

  \savedanchor{\BaseAnortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@y=0.30\pgf@ya
    \pgf@x=0.12\pgf@xa
  }

  % Maybe I don't need this savedanchor
  \savedanchor{\MiddleAntennasouth}{
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0pt
    \pgf@y=0.29\pgf@ya
  }

  \savedanchor{\AntennaConnectorsouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=-0.5\pgf@xa
    \pgf@y=0.38\pgf@ya
  }

  \savedanchor{\AntennaConnectornortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0.5\pgf@xa
    \pgf@y=0.42\pgf@ya
  }

  \savedanchor{\MiddleAntennasouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=-0.15\pgf@xa
    \pgf@y=0.29\pgf@ya
  }

  \savedanchor{\MiddleAntennanortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0.15\pgf@xa
    \pgf@y=0.5\pgf@ya
  }

  \savedanchor{\LeftAntennasouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=-0.5\pgf@xa
    \pgf@y=0.29\pgf@ya
  }

  \savedanchor{\LeftAntennanortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=-0.25\pgf@xa
    \pgf@y=0.5\pgf@ya
  }

  \savedanchor{\RightAntennasouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0.25\pgf@xa
    \pgf@y=0.29\pgf@ya
  }

  \savedanchor{\RightAntennanortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0.5\pgf@xa
    \pgf@y=0.5\pgf@ya
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit anchor border from UserTerminal xxxxxxxxxxxxxxxxxxxx
  \inheritanchorborder[from=UserTerminal]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit normal anchors from UserTerminal xxxxxxxxxxxxxxxxxxx
  % We define the savedanchors "northeast" and "southwest". With these two
  % defined we can inherit code for the regular anchors from the
  % UserTerminal shape (even thought the northeast and southwest saved anchors
  % in the UserTerminal shape are different from ours).
  \inheritanchor[from=UserTerminal]{center}
  \inheritanchor[from=UserTerminal]{north}
  \inheritanchor[from=UserTerminal]{east}
  \inheritanchor[from=UserTerminal]{south}
  \inheritanchor[from=UserTerminal]{west}
  \inheritanchor[from=UserTerminal]{north east}
  \inheritanchor[from=UserTerminal]{north west}
  \inheritanchor[from=UserTerminal]{south west}
  \inheritanchor[from=UserTerminal]{south east}
  \inheritanchor[from=rectangle]{text}
  \anchor{antenna right}{
    \northeast
    \pgfmathsetlength\pgf@y{0.8*\pgf@y}
  }
  \anchor{antenna left}{
    \northeast
    \pgfmathsetlength\pgf@y{0.8*\pgf@y}
    \pgfmathsetlength\pgf@x{-\pgf@x}
  }
  \anchor{antenna center}{
    \northeast
    \pgfmathsetlength\pgf@y{0.8*\pgf@y}
    \pgfmathsetlength\pgf@x{0}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Draw the "behind background" xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % The base of the antenna will be in the behindbackgroundpath while the
  % antennas will be in the backgroundpath.
  \behindbackgroundpath{
    % Scope for the Base
    \begin{pgfscope}
      % Draw the bottom base
      \pgfpathrectanglecorners
      {\BaseAsouthwest}
      {\BaseAnortheast}

      \pgfusepath{stroke,fill}
    \end{pgfscope}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Draw the background xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % The base of the antenna will be in the behindbackgroundpath while the
  % antennas will be in the backgroundpath. The main reason for this
  % separation is that this code here will be inherited in the
  % "BaseStation" shape that we will define later.
  \backgroundpath{
    % Scope for the antenna connector
    \begin{pgfscope}
      % Draw Antenna connector
      \pgfpathrectanglecorners
      {\AntennaConnectorsouthwest}
      {\AntennaConnectornortheast}

      \pgfusepath{stroke,fill}
    \end{pgfscope}

    % Scope for the antennas
    \begin{pgfscope}
      % Draw the middle antenna
      \pgfpathrectanglecorners
      {\MiddleAntennasouthwest}
      {\MiddleAntennanortheast}

      % Draw the Left antenna
      \pgfpathrectanglecorners
      {\LeftAntennasouthwest}
      {\LeftAntennanortheast}

      % Draw the Right antenna
      \pgfpathrectanglecorners
      {\RightAntennasouthwest}
      {\RightAntennanortheast}

      \pgfusepath{stroke,fill}
    \end{pgfscope}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
}
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx END xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx


% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx BaseStation Shape xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
\pgfdeclareshape{BaseStation}{

  % xxxxxxxxxx Define savedanchors xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % Inherit all savedanchors from BaseStationSimple.
  \inheritsavedanchors[from=BaseStationSimple]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxx Define savedanchors specific to the BaseStation shape xxxxxxxxxxx
  \savedanchor{\BaseAsouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@y=-0.5\pgf@ya
    \pgf@x=-0.2\pgf@xa
  }

  \savedanchor{\BaseAnortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@y=-0.05\pgf@ya
    \pgf@x=0.2\pgf@xa
  }

  \savedanchor{\BaseBsoutheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@y=-0.05\pgf@ya
    \pgf@x=0.15\pgf@xa
  }

  \savedanchor{\BaseBnorthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@y=0.15\pgf@ya
    \pgf@x=-0.15\pgf@xa
  }

  \savedanchor{\BaseCsouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@y=0.15\pgf@ya
    \pgf@x=-0.1\pgf@xa
  }

  \savedanchor{\BaseCnortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@y=0.30\pgf@ya
    \pgf@x=0.1\pgf@xa
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit anchor border from BaseStationSimple xxxxxxxxxxxxxxx
  \inheritanchorborder[from=BaseStationSimple]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit normal anchors from BaseStationSimple xxxxxxxxxxxxxx
  % We define the savedanchors "northeast" and "southwest". With these two
  % defined we can inherit code for the regular anchors from the
  % BaseStationSimple shape (even thought the northeast and southwest saved anchors
  % in the BaseStationSimple shape are different from ours)..
  \inheritanchor[from=BaseStationSimple]{center}
  \inheritanchor[from=BaseStationSimple]{north}
  \inheritanchor[from=BaseStationSimple]{east}
  \inheritanchor[from=BaseStationSimple]{south}
  \inheritanchor[from=BaseStationSimple]{west}
  \inheritanchor[from=BaseStationSimple]{north east}
  \inheritanchor[from=BaseStationSimple]{north west}
  \inheritanchor[from=BaseStationSimple]{south west}
  \inheritanchor[from=BaseStationSimple]{south east}
  \inheritanchor[from=BaseStationSimple]{antenna right}
  \inheritanchor[from=BaseStationSimple]{antenna left}
  \inheritanchor[from=BaseStationSimple]{antenna center}
  \inheritanchor[from=rectangle]{text}
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Draw the "behind background" xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \behindbackgroundpath{
    % Scope for the Base
    \begin{pgfscope}
      % Draw the bottom base
      \pgfpathrectanglecorners
      {\BaseAsouthwest}
      {\BaseAnortheast}

      % Draw the middle base
      \pgfpathrectanglecorners
      {\BaseBsoutheast}
      {\BaseBnorthwest}

      % Draw the bottom base
      \pgfpathrectanglecorners
      {\BaseCsouthwest}
      {\BaseCnortheast}

      \pgfusepath{stroke,fill}
    \end{pgfscope}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxx Inherit the background path from BaseStationSimple xxxxxxxxxxx
  \inheritbackgroundpath[from=BaseStationSimple]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
}
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx END xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

\makeatother

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "testbasestation.tex"
%%% TeX-PDF-mode: t
%%% End:


==> figs/vehicles.tex <==
\usetikzlibrary{backgrounds}

\tikzset{
    olwyn/.style={circle, draw, line width=#1*.8pt, minimum width=#1*5pt, inner sep=0pt, fill=gray!75},
    pics/tram/.style={
        code={
          \path [draw, line width=#1*.8pt, fill=white]
          coordinate (tram) ++(-.2*#1,#1*2.75pt) node (w1) [olwyn=#1] {}
                  ++(#1*.425,0) node (w2) [olwyn=#1] {}
                  ++(#1*.425,0) node (w3) [olwyn=#1] {};
          \path [draw, fill=white, line width=#1*.4pt]
                (w1) circle (#1*1pt)
                (w2) circle (#1*1pt)
                (w3) circle (#1*1pt);
          \path [draw, fill=white, line width=#1*.4pt]
                (tram) ++(-.4*#1,#1*1.5pt) coordinate (t1) |- ++(#1*1.25,#1*.35) coordinate (t2) |- (w3.south east -| w3.east) |- (w3.west) |- (w2.south east -| w2.east) |- (w2.west) |- (w1.south east -| w1.east) |- (w1.west) -- (w1.south west -| w1.west) -| cycle
                (t1 -| t2) ++(-.05*#1pt,#1*4pt) coordinate (t3) |- ++(-.175*#1,#1*.175) coordinate (t4) |- cycle
                (t3 -| t4) ++(-.5*#1pt,0) |- ++(-.25*#1,.175*#1) coordinate (t5) |- cycle
                (t3 -| t5) ++(-.5*#1pt,0) |- ++(-.25*#1,.175*#1) coordinate (t6) |- cycle
                (t3 -| t6) ++(-.5*#1pt,0) |- ++(-.25*#1,.175*#1) coordinate (t7) |- cycle
                (t3 -| t7) ++(-.5*#1pt,0) |- ++(-.25*#1,.175*#1) coordinate (t8) |- cycle;
          \scoped [on background layer] \fill [color=white] (t3) rectangle (t8);
        }
    }
}

\tikzset{
    pics/bot/.style={
        code={
            \draw[draw=black,fill=white,rounded corners=0.4ex*#1,line width=#1*.4pt] (0.15*#1,.05*#1) rectangle (0.65*#1,0.25*#1);
            \draw[draw=black,fill=gray!50,thick] (0.3*#1,.05*#1) circle (.05*#1);
            \draw[draw=black,fill=gray!50,thick] (0.5*#1,.05*#1) circle (.05*#1);    
            \draw[draw=black,fill=gray!80,semithick] (0.3*#1,.05*#1) circle (.04*#1);
            \draw[draw=black,fill=gray!80,semithick] (0.5*#1,.05*#1) circle (.04*#1);
            \draw[line width=#1*.8pt] (0.25*#1,0.25*#1) -- (0.25*#1,0.42*#1);
            \draw[fill=black] (0.25*#1,0.42*#1) circle (0.03*#1);
        }
    }
}

\tikzset{
    pics/car/.style={
        code={
                \draw[draw=black,fill=white,rounded corners=.4ex*#1,line width=#1*0.80pt] 
                (1.5*0.20*#1,.5*0.20*#1) -- ++
                (0*0.20*#1,1*0.20*#1) -- ++
                (1*0.20*#1,0.3*0.20*#1) --  ++
                (3*0.20*#1,0*0.20*#1) -- ++
                (1*0.20*#1,0*0.20*#1) -- ++
                (0*0.20*#1,-1.3*0.20*#1) -- 
                (1.5*0.20*#1,.5*0.20*#1) -- cycle;
                \draw[rounded corners=0.4ex*#1,fill=white,line width=#1*.4pt]  
                    (2.5*0.20*#1,1.8*0.20*#1) -- ++
                    (1*0.20*#1,0.7*0.20*#1) -- ++
                    (1.6*0.20*#1,0*0.20*#1) -- ++
                    (0.6*0.20*#1,-0.7*0.20*#1) -- 
                    (2.5*0.20*#1,1.8*0.20*#1);
                \draw[thick]  (0.84*#1,0.36*#1) -- (0.84*#1,0.50*#1);
                \draw[draw=black,fill=gray!50,line width=#1*0.400pt] (2.75*0.20*#1,.5*0.20*#1) circle (.5*0.20*#1);
                \draw[draw=black,fill=gray!50,line width=#1*0.40pt] (5.5*0.20*#1,.5*0.20*#1) circle (.5*0.20*#1);
                \draw[draw=black,fill=gray!80,line width=#1*0.20pt] (2.75*0.20*#1,.5*0.20*#1) circle (.4*0.20*#1);
                \draw[draw=black,fill=gray!80,line width=#1*0.20pt] (5.5*0.20*#1,.5*0.20*#1) circle (.4*0.20*#1);
        }
    }
}
